Saddle Flow Dynamics: Observable Certificates and Separable Regularization

This paper proposes a certificate, rooted in observability, for asymptotic convergence of saddle flow dynamics of convex-concave functions to a saddle point. This observable certificate directly bridges the gap between the invariant set and the equilibrium set in a LaSalle argument, and generalizes conventional conditions such as strict convexity-concavity and proximal regularization. We further build upon this certificate to propose a separable regularization method for saddle flow dynamics that makes minimal requirements on convexity-concavity and yet still guarantees asymptotic convergence to a saddle point. Our results generalize to saddle flow dynamics with projections on the vector field and have an immediate application as a distributed solution to linear programs.

==> Saddle_Flow_Dynamics_ACC'21_update/edits.tex <==
\usepackage{ifthen}
\newboolean{showcomments}
\setboolean{showcomments}{true}
\usepackage[usenames,dvipsnames]{color}
\usepackage{todonotes}

\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}

%ADD CITES
\newcommand{\addcite}[0]{\ifthenelse{\boolean{showcomments}}
{\textcolor{purple}{(add cite(s)) }}{}}%

% Comments
\newcommand{\enrique}[1]{  \ifthenelse{\boolean{showcomments}}
{\todo[inline,color=bleudefrance]{Enrique: #1}}{}}
\newcommand{\emmargin}[1]{\ifthenelse{\boolean{showcomments}}{\marginpar{\color{bleudefrance}\tiny EM: #1}}{}}


%Edits to be highlighted
\newboolean{showedits}
\setboolean{showedits}{false}
\usepackage[markup=underlined]{changes}
\definechangesauthor[color=bleudefrance]{EM}
\newcommand{\aem}[1]{
\ifthenelse{\boolean{showedits}}
{\added[id=EM]{#1}}
{\!#1\hspace{-4.75pt}}
}
\newcommand{\repem}[2]{
\ifthenelse{\boolean{showedits}}
{\replaced[id=EM]{#1}{#2}}
{\!#1\hspace{-4.75pt}}
}
\newcommand{\dem}[1]{
\ifthenelse{\boolean{showedits}}
{\deleted[id=EM]{#1}}
{}
}
%\listoftodos[{\color{red}\textbf{List of comments/suggestions}}]


==> Saddle_Flow_Dynamics_ACC'21_update/writing_pcyou.tex <==

\usepackage{epsfig, latexsym, times, bbm}
\usepackage{color}
\usepackage{colortbl}
\usepackage{array}
\usepackage{cite}

\usepackage{amsmath}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{url}
\usepackage{comment}

\let\proof\relax 
\let\endproof\relax
\usepackage{amsthm}


\usepackage{multirow}
\def\UrlBreaks{\do\/\do-}

\usepackage{bbding}
\usepackage{amsfonts}
\usepackage{cases}


\usepackage{algorithmic}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{verbatim}
\usepackage{enumerate}

\usepackage{booktabs}
\usepackage[linesnumbered,ruled,longend]{algorithm2e}
\usepackage{textcomp}
\usepackage{subeqnarray}
\usepackage{dsfont,optidef}

\usepackage{subfig}





%% added
\def\ba{\begin{align}}
	\def\ea{\end{align}}
\newcommand{\beq}{\begin{equation}}
	\newcommand{\eeq}{\end{equation}}
\newcommand{\bq}{\begin{eqnarray}}
	\newcommand{\eq}{\end{eqnarray}}
\newcommand{\bqn}{\begin{eqnarray*}}
	\newcommand{\eqn}{\end{eqnarray*}}
\newcommand{\bee}{\begin{enumerate}}
	\newcommand{\eee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
	\newcommand{\ei}{\end{itemize}}
\newcommand{\bseq}{\begin{subequations}}
\newcommand{\eseq}{\end{subequations}}
\renewcommand{\qed}{\hfill{$\blacksquare$}}
\newcommand{\ii}{\textbf{i}}






\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}
\newcommand{\cell}[3]{\parbox[c][#2][c]{#1}{\makebox[#1]{#3}}}

\renewcommand\thepage{}
\renewcommand{\arraystretch}{1.3}

% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\allowdisplaybreaks






%%%%%%%%%%%%%%%%%%%%
%% Math Operators %%
%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\nullsp}{Null}
\DeclareMathOperator{\supprt}{Supp}
\DeclareMathOperator{\asc}{asc}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\rint}{rint}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\proj}{Pr}


% Custom made commands and environments
\newcommand*\mbf[1]{\ensuremath{\mathbf{#1}}}  % creates a bold symbol
\newcommand*\dt[0]{\frac{d}{dt}} % time derivative d/dt
\newcommand*\mc[0]{\mathcal}                                                  		% abbreviation for \mathcal
\newcommand*\mbb[0]{\mathbb}                                                  		% abbreviation for \mathbb
\newcommand{\subscr}[2]{{#1}_{\textup{#2}}}
\newcommand{\until}[1]{\{1,\dots,#1\}}
\newcommand{\tg}[0]{\color{Gray}}
% matrix operations
\newcommand*\Ker[0]{\mbox{Ker}} 
\newcommand*\Img[0]{\mbox{Im}} 
\newcommand*\Rank[0]{\mbox{rank}} 
\newcommand*\Span[0]{\mbox{span}} 
\newcommand*\Dim[0]{\mbox{dim}} 
\newcommand*\diag[0]{\mbox{diag}} 
\newcommand*\blockdiag[0]{\mbox{blockdiag}}



\newcommand{\R}{\mathbb{R}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\dd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\dsqd}[2]{\frac{\partial^2}{\partial #1\partial #2}}






%%%%%%%%%%%%%%%%%%%%
%%% Environments %%%
%%%%%%%%%%%%%%%%%%%%

\newtheorem*{remark}{Remark}
\newtheorem{theorem}{{Theorem}}%[section]
\newtheorem{lemma}[theorem]{{Lemma}}
\newtheorem{definition}{{Definition}}
\newtheorem{corollary}[theorem]{{Corollary}}
\newtheorem{proposition}[theorem]{{Proposition}}
\newtheorem{problem}{{Problem}}
% \newtheorem{remark}{{Remark}}
% \newtheorem*{remark}{{Remark}}
\newtheorem{assumption}{{Assumption}}
\newtheorem{example}{{Example}}
\newtheorem{claim}{{Claim}}



